A Search for Z=-1 Dark Matter Annihilation Products in Cosmic Rays with AMS-01

The majority of mass in the universe has not been observed optically and is termed dark matter. The supersymmetric neutralino provides an interesting dark matter candidate, which may self-annihilate in our galaxy, producing particles visible in the cosmic ray spectrum. During a ten day space shuttle flight, the AMS-01 detector recorded over 100 million cosmic ray events. This analysis searches for the products of neutralino annihilation in the AMS-01 Z=-1 spectrum, and uses the results to place limits on which supersymmetric and dark matter halo distribution models are compatible.

==> Bibliography.tex <==
\begin{thebibliography}{0}
%the pdg's summary of dark matter
\bibitem{ref:pdgdarkmatter}
W.-M. Yao et al., Journal of Physics G 33, 1 (2006) [pdg.lbl.gov]
%use this when referring to the whole pdg
\bibitem{ref:pdgstraightup} TODO the pdg
%CDMS spin independent paper
\bibitem{ref:cdmsnospin} D.S. Akerib et al. Limits on spin-independent WIMP-nucleon interactions from the two-tower run of the Cryogenic Dark Matter Search Phys.Rev.Lett. 96 (2006) 011302  [astro-ph/0509259]
%supercdms proposal
\bibitem{ref:supercdms} D.S. Akerib. et al. "The SuperCDMS proposal for dark matter detection" NIM A, Volume 559, Issue 2  , 15 April 2006, Pages 411-413 
% XENON paper (TODO find a better one than this)
\bibitem{ref:XENON} E. Aprile.  "XENON: A 1 Tonne Liquid Xenon Experiment For a Sensitive Dark Matter Search".  [astro-ph/0207670]
%a PICASSO paper
\bibitem{ref:PICASSO} L. A. Hamel et al. "A superheated droplet detector for dark matter search" NIM A Volume 388, Issues 1-2  , 21 March 1997, Pages 91-99%a DRIFT paper TODO Get this
\bibitem{ref:DRIFT} G.J. Alner et al. "The DRIFT-II dark matter detector: Design and commissioning", NIM A 555 (2005) 173-183.
%a heat positron paper
\bibitem{ref:HEAT1} S.~W.~Bartwick et al. THE ENERGY SPECTRA AND RELATIVE ABUNDANCES OF ELECTRONS AND POSITRONS IN THE GALACTIC COSMIC RADIATION. THE ASTROPHYSICAL JOURNAL, 498 : 779È789, 1998 May 10
%generic EGRET DM paper
\bibitem{ref:EGRET1} W. de Boer, et al. arXiv:astro-ph/0508617 v1 29 Aug 2005 EGRET Excess of Diffuse Galactic Gamma Rays as Tracer of Dark Matter Astron. Astrophys. 44 (2005) L51 [arxiv:astro-ph/0508617]
%an icecube paper TODO find a better paper that talks about 
%                you can look at neutrinos in the sun with this
\bibitem{ref:ICECUBE} IceCube Collaboration "First Year Performance of The Ice Cube Neutrino Telescope" Astropart.Phys. 26 (2006) 155-173
%my Astro 2 book, good with DM distributions
\bibitem{ref:galaxybook} J. Binney and S. Tremaine, Galactic Dynamics (Princeton University Press, Princeton, NJ, 1994). %hard copy sitting on my desk
% Zwicky's  paper (the english one, not the german one)
\bibitem{ref:zwicky} F. Zwicky.  On the Masses of Nebulae and Of Clusters of Nebulae  apj,Vol 86:3 1937  217-246
%A semi-recent measure of the dark matter content of the coma cluster.
%don't let the title fool you, there's stil a lot of DM there
\bibitem{ref:newcoma} L. L. Cowie, M. Henriksen, and R. Mushotzky, Are the virial masses of clusters smaller than we think? The Astrophysical Journal, volume 317 (1987), page 593 
%the official wmap 3 year paper, I think
\bibitem{ref:wmap} D.N. Spergel et al. Wilkinson Microwave Anisotropy Probe (WMAP) Three Year Results: Implications for Cosmology. 2006.  ApJ.  [astro-ph/0603449]
% has a bunch of galactic rotation curves
% kind of amusingly though, it favors modified gravity over dark matter
\bibitem{ref:GalaxyRotCurves} K.G. Begeman et al. Extended rotation curves of spiral galaxies: dark haloes and modified dynamics. Mon. Not. R. Astr. Soc (1991) 249, 523-537
%huge long paper on susydark matter
\bibitem{ref:ssdm} G. Jungman et al. Supersymmetric Dark Matter. Physics Reports 267. (1996) 195-373
%the axion experiment  that gp now works on
\bibitem{ref:axions} S.J. Asztalos et al., Improved rf cavity search for halo axions.  Phys. Rev. D 69, 011101(R) (01 Jan 2004)
%where I get the claim that local density is greater than 0.25 GeV
\bibitem{ref:dmdensity}
M. Kamionkowski and A. Kinkhabwala. Galactic halo models and particle dark-matter detection.  Phys. Rev. D.  57. num6 3256-3263
% 
\bibitem{ref:bertclumps} E. Bertschinger. Effects of cold dark matter decoupling and pair annihilation on cosmological perturbations. arxiv: astro-ph/0607319 2006
%
\bibitem{ref:caustics} R. Mohayaee and S. Shandarin. Gravitational cooling and density profile near caustics in collisionless dark matter haloes.  arxiv: astro-ph/0503163
% here is where they get those funny greens functions that they can't reproduce
\bibitem{ref:galpropgreens}  I.V. Moskalenko and A.W. Strong, Positrons from particle dark-matter annihilation in the Galactic halo: Propagation Green’s functions, Phys. Rev. D., Vol 60, 1999 
%fermi talks fermi accelleration
\bibitem{ref:fermi} E. Fermi.  On the Origin of the Cosmic Radiation.  Physical Review, 75(8):1169-1174, April 1949.
%shock acceleration
\bibitem{ref:shocks} R.D. Blanford and J.P. Ostriker.  Particle Acceleration by Astrophysical Shocks. The Astrophysical Journal, 221:L29-L32, April 1978.
%Gianpaolo's thesis
\bibitem{ref:gpthesis} G.P. Carosi. \newblock {\em {A Search for Signatures of Dark Matter in the AMS-01 Electron and Antiproton Spectrum}}.  PhD dissertation, MIT, Physics Department, January 2006.
%The paper allegedly gives the isothermal halo distribution (cored) Look for it
%again in it
\bibitem{ref:nfw} J.F. Navarro, C.S. Frenk, and S.D.M. White. \newblock {A Universal Density Profile From Hierarchical Clustering} {\it Astroph. J.} {\bf 490} 493 (1997)
%A galprop paper
\bibitem{ref:galprop} I.V. Moskalenko and A.W. Strong. \newblock {Production and Propagation of Cosmic-Ray Positrons and Electrons}. {\it Astroph. J.} {\bf 493},694-707 (1998).
%another galprop paper
\bibitem{ref:thegalprop} I.V. Moskalenko and A.W. Strong. Propagation of Cosmic Ray Nucleons in the galaxy.  ApJ.  509:212--228 (1998)
%a review of susy at the LHC
\bibitem{ref:lhcsusy} D.P. Roy.  Higgs and SUSY Searches at LHC: An Overview. Acta Phys.Polon. B34 (2003) 3417-3440 hep-ph/0303106
%the AMS01 physics report
\bibitem{ref:AMS01} M.~Aguilar et~al. (AMS~Collaboration). \newblock {The Alpha Magnetic Spectrometer (AMS) on the International Space Station: Part I - Results from the Test Flight on the Space Shuttle}. \newblock {\em Physics Reports}, 366(6):331--405, 2002.
%re the AMS01 Magnet
\bibitem{ref:AMS01Mag} S.~Ahlen et~al. \newblock {An Antimatter Spectrometer in Space}. \newblock {\em Nuclear Instruments and Methods A}, 350:351--367, 1994.
%re AMS01 event reconstruction
\bibitem{ref:Reconstruction}
Vitaly Choutko. \newblock {Selected AMS01 Reconstruction Software Issues}. \newblock AMS Internal Presentation, January 2003.
%re AMS01 tracker
\bibitem{ref:AMS01Tracker} J.~Alcaraz et~al. \newblock {A Silicon microstrip tracker in space: Experience with the AMS silicon tracker on STS-91}. \newblock {\em Il Nouvo Cimento}, 112A(11):1325--1344, 1999.
%re AMS01 TOF
\bibitem{ref:AMS01TOF} L.~Baldini et~al. \newblock {The AMS-01 Time of Flight System}. \newblock In {\em 7th Int. Conf. on Advanced Technology and Particle Physics},   2001.
%re AMS01 TOF
\bibitem{ref:AMS01TOF2} D.~Alvisi et~al. \newblock {A high resolution, low power time-of-flight system for the space experiment AMS}. \newblock {\em Nuclear Instruments and Methods in Physics Research A}, 437:212--221, 1999. 
%Christinziani's thesis
\bibitem{ref:CristHardName} Markus Cristinziani. \newblock {\em {Search for Heavy Antimatter and Energetic Photons in Cosmic Rays with the AMS-01 Detector in Space}}. \newblock {PhD} dissertation, University of Geneva, Department of Physics, February 2002.
%re Fast Fit Algorithm
\bibitem{ref:FastFit} J.C. Hart and D.H. Saxon. \newblock {Track and Vertex Fitting in an Inhomogeneous Magnetic Field}. \newblock {\em NIM}, 220:309--326, 1984.
%PDG section on particles passing through materials
\bibitem{ref:PDGPassage} TODO is this the right way to cite this Particle~Data Group. \newblock {Review of Particle Physics: Passage of Particles Through Matter}. \newblock {\em Physics Letters B}, 592:242--253, 2004.
%re AMS01 montecarlo
\bibitem{ref:Simulation} Vitaly Choutko. \newblock {AMS Simulation Software Overview}. \newblock AMS Internal Presentation, January 1997. % TODO FIND
%re AMS01 Data Format
\bibitem{ref:DataFormats} Mike Capell and Alexei Lebedev. \newblock {AMS Data Formats}. \newblock AMS Internal Report, October 1997. % TODO FIND
% This seems useful
\bibitem{ref:Fits} Vitaly Choutko. \newblock {On the Alignment of the AMS SI Tracker by Means of Charged  Particles}. \newblock AMS Internal Paper, January 1996.
%re Acceptance and such
\bibitem{ref:Telescope} J.D. Sullivan. \newblock {Geometrical Factor and Directional Response of Single and Multi-Element Particle Telescopes}. \newblock {\em NIM}, 95:5--11, 1971.
%trigger design
\bibitem{ref:trigger} Vitaly Choutko. AMS Trigger During Shuttle Flight. AMS Internal Presentation, May 1998.
%re trigger systematic errors
\bibitem{ref:TriggerSystematics} Vitaly Choutko. \newblock {AMS Proton Trigger Acceptance Study}. \newblock AMS Internal Presentation, June 1999.
%re my minuit fitting
\bibitem{ref:Minuit} F.~James. \newblock {\em {MINUIT: Function Minimization and Error Analysis}}. \newblock CERN Computing and Networks Division, Geneva, Switzerland, version 94.1 edition, August 1998. % TODO I have hard copy, find ecopy
%Pythia Paper
\bibitem{ref:Pythia} Torbj$\ddot{o}$rn~Sj$\ddot{o}$strand et~al. \newblock {High-energy-physics event generation with PYTHIA 6.1}. \newblock {\em Computer Physics Communications}, 135:238--259, 2001. % TODO FIND, I only have manual
%Caprice electron paper
\bibitem{ref:capriceelectrons} M. Boezio et~al. \newblock{The Cosmic-Ray Electron and Positron Spectra Measured at 1 AU During Solar Minimum Activity}. \newblock{\it Astroph. J.} 532:653--669 (2000)
%Caprice proton paper
\bibitem{ref:capriceprotons} M. Boezio et~al. \newblock{The Cosmic-Ray Proton and Helium Spectra Between 0.4 and 200 GV}. \newblock{\it Astroph. J.} 518:457--472 (1999)
%galprop paper where they get injection indicies (maybe also cite for SM choice)
\bibitem{ref:galpropparams} I. Moskalenko et~al. \newblock{Secondary Antiprotons and Propagation of Cosmic Rays in the Galaxy and Heliosphere} \newblock{\it Astroph. J.} 565:280--296 (2002)
%use this for emails exchanged with moskalenko
\bibitem{ref:moskocommun} I. Moskalenko, personal communications
%-The- definitive force field approximation Solar Modulation paper
\bibitem{ref:thesmpaper} L.J. Gleeson and W.I. Axford. \newblock{Solar Modulation of Galactic Cosmic Rays} \newblock{\it Astroph. J.} 154:1011--1026 (1968)
%dark susy suggested paper
\bibitem{ref:darksusy} P. Gondolo, J. Edsjö, P. Ullio, L. Bergstöm, M. Schelke and E.A. Baltz, JCAP 0407 (2004) 008 [astro-ph/0406204]
%isasjet paper to reference, since darksusy uses isasugra from it
\bibitem{ref:isasugra} F.E. Paige, S.D. Protopescu, H. Baer, X. Tata, [arXiv:hep-ph/0312045]
%longair's High Energy Astrophysics book.  Mostly a primer on high energy
%interactions, with a bit of plasma physics thrown in for good measure
\bibitem{ref:logairv1} M. Longair.  High Energy Astrophysics. Vol. 1: Particles, photons, and their detection. Cambridge University Press.  1992.  Cambridge. %hard copy sitting on my desk.  I think it was stolen from the physics reading room before my time.  return it when I graduate
%an ancient book where stormer lays it out for the geomagnitic cutoff
\bibitem{ref:stormer} C. St{\o}rmer. The polar aurora. Oxford, Clarendon Press, 1955. %I read this and took notes, don't have photocopy of it I think, don't know where notes are TODO find notes and put them someplace safe
%pdg on cosmic rays
\bibitem{ref:pdgcray} TODO PDG Cosmic rays review
%particle astrophysics the book, in building 44
\bibitem{ref:partastrobook} D. Perkins. Particle Astrophysics, volume 1 of Oxford Master Series in Particle Physics, Astrophysics, and Cosmology.  Oxford university Press, Oxford, UK, first edition 2003. %have photocopy of relevant section
%susy points updated from wmap
\bibitem{ref:sspoints} M. Battaglia et al. Proposed Post-LEP Benchmarks for Supersymmetry.  June 2001. [hep-ph/0106204]
\bibitem{ref:sspointsupdated} M. Battaglia et al.  Updated Post-WMAP Benchmarks for Supersymmetry. June 2003.  [hep-ph/0306219]
%a pointer to the atc
\bibitem{ref:atc} D. Barancourt et al. The AMS-01 Aerogel Threshold Cherenkov counter. Nuclear Instruments and Methods in Physics Research A 465 (2001) 306–317
%the susy book from the susy course at MIT (better than D. Freedman's notes)
\bibitem{ref:susybook} J. Terning. Modern Supersymmetry. Oxford, Oxford University Press, 2006.
%pdg entry on susy (theory)
\bibitem{ref:pdgsusy} TODO PDG SUSY THEORY
%heat paper that gives some susy models
\bibitem{ref:HEAT2} E. Baltz and J. Edsj\"o. Positron Propagation and Fluxes from Neutralino Annihilation in the Halo, (look up, it's in Phys. Rev. D, written on printed copy)
%EGRET mSugra paper
\bibitem{ref:EGRET2} W. de Boer et al. The supersymmetric interpretation of the EGRET excess of diffuse Galactic gamma rays. arxiv:hep-ph/0511154 Phys.Lett. B636 (2006) 13-19 
%BESS paper
\bibitem{ref:BESS3} S. Orito, et al.  Precision Measurement of Cosmic-Ray Antiproton Spectrum Phys. Rev. Let. 84 (2000) 1078.
%Comparison to cdms-II and points
\bibitem{ref:directpoints} J. Ellis et al. Update on the Direct Detection of Supersymmetric Dark Matter Phys.Rev. D71 (2005) 095007, arxiv:hep-ph/0502001
%this website generates sweet-ass plots of direct detection limits
\bibitem{ref:directplotgen} R. Gaitskell, V. Mandic, and J. Filippini.  "Direct Detection of WIMP Dark Matter, Sensitivity Plots", http://dmtools.berkeley.edu/limitplots/
\bibitem{ref:talkgondolo} Paolo Gondolo. 2006. Private Communication.
\bibitem{ref:BESS1} T.Maeno et al.  Successive Measurements of Cosmic-Ray
Antiproton Spectrum in a Positive Phase of the Solar Cycle, [astro-ph/0010381]
\bibitem{ref:BESS2} Y.Asaoka. Measurements of Cosmic-ray Low-energy Antiproton and Proton Spectra in a Transient Period of the Solar Field Reversal. [astro-ph/0109007]
\bibitem{ref:earlyclumps} J.Diemand et al. Earth-mass dark-matter haloes as the first structures in the early Universe, Nature 433 (2005) 389-391

\end{thebibliography} 

